A Deep Inference System for Differential Linear Logic

Differential linear logic (DiLL) provides a fine analysis of resource consumption in cut-elimination. We investigate the subsystem of DiLL without promotion in a deep inference formalism, where cuts are at an atomic level. In our system every provable formula admits a derivation in normal form, via a normalization procedure that commutes with the translation from sequent calculus to deep inference.

==> eptcsdata.tex <==
\providecommand{\firstpage}{26}
\providecommand{\publicationstatus}{U. Dal Lago and V. de Paiva (Eds.) Second Joint International\\ Workshop on Linearity \& Trends in Linear Logic and Applications.\\
EPTCS 353, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.353.2}{10.4204/EPTCS.353.2}}
\pdfoutput=1

